Towards Effective Top-N Hamming Search via Bipartite Graph Contrastive Hashing

Searching on bipartite graphs serves as a fundamental task for various real-world applications, such as recommendation systems, database retrieval, and document querying. Conventional approaches rely on similarity matching in continuous Euclidean space of vectorized node embeddings. To handle intensive similarity computation efficiently, hashing techniques for graph-structured data have emerged as a prominent research direction. However, despite the retrieval efficiency in Hamming space, previous studies have encountered catastrophic performance decay. To address this challenge, we investigate the problem of hashing with Graph Convolutional Network for effective Top-N search. Our findings indicate the learning effectiveness of incorporating hashing techniques within the exploration of bipartite graph reception fields, as opposed to simply treating hashing as post-processing to output embeddings. To further enhance the model performance, we advance upon these findings and propose Bipartite Graph Contrastive Hashing (BGCH+). BGCH+ introduces a novel dual augmentation approach to both intermediate information and hash code outputs in the latent feature spaces, thereby producing more expressive and robust hash codes within a dual self-supervised learning paradigm. Comprehensive empirical analyses on six real-world benchmarks validate the effectiveness of our dual feature contrastive learning in boosting the performance of BGCH+ compared to existing approaches.

==> analysis.tex <==
\section{Theoretical Proofs and Analyses}
\label{sec:discuss}
\addtocounter{thm}{-1}

% \subsection{Theorem Proofs}
% \label{sec:dispersion}

% \input{fd_analysis}



% \begin{thm}[\textbf{Hamming Distance Matching}]
% Given two hash codes, we have $(\alpha_x\emb{Q}_u)^\mathsf{T} \cdot (\alpha_y\emb{Q}_y) = \alpha_x\alpha_y (d - 2D_{H}(\emb{Q}_x, \emb{Q}_y))$.
% \end{thm} 

% \begin{proof}
% % Since the encoded hamming space is $\{-1,1\}^d$, we have:
% \begin{equation}
% \begin{aligned}
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}
% &\emb{Q}_x^\mathsf{T} \cdot \emb{Q}_y \\ 
% &= \big|\{ i|(\emb{Q}_{x})_i = (\emb{Q}_{y})_i = 1\}\big| +  \big|\{ i|(\emb{Q}_{x})_i = (\emb{Q}_{y})_i = -1\}\big| \\ 
% & -  \big|\{ i|(\emb{Q}_{x})_i \neq (\emb{Q}_{y})_i\}\big|\\
% & = d - 2 \cdot \big|\{ i|(\emb{Q}_{x})_i \neq (\emb{Q}_{y})_i\}\big|  = \underline{d - 2D_{H}(\emb{Q}_x, \emb{Q}_y))},\\
% \end{aligned}
% \end{equation}%
% which completes the proof.
% \end{proof}


% \subsection{Complexity Analysis}
% \label{sec:complexity}


% \subsubsection{\textbf{Training Time Complexity.}}
\textbf{Training time complexity.}
As shown in Table~\ref{tab:train_time}, $|\mathcal{E}|$, $B$, $s$, and $n$ are the edge number, batch size, numbers of train iterations and Fourier Series decomposition terms.
(1) The time complexity of the graph normalization, i.e., $\emb{D}^{-\frac{1}{2}} \emb{A} \emb{D}^{-\frac{1}{2}}$, is $O(2|\mathcal{E}|)$.
(2) Before the graph convolution, we first conduct the feature dispersion only for the initial node embeddings, e.g., $\emb{V}_x^{(0)}$, which takes $O(\frac{2csK|\mathcal{E}|^2}{B})$ complexity.
In our experiment, hyper-parameter $K \leq 3$.
(3) In graph convolution, the time complexity is $O(\frac{2csL|\mathcal{E}|^2}{B})$, where $L \leq 4$ is a common setting~\cite{lightgcn,ngcf,kipf2016semi,graphsage} to avoid \textit{over-smoothing}~\cite{li2019deepgcns}.
(4) As for the loss computation, \model~takes $O\big(2sc|\mathcal{E}|\big)$ to compute $\mathcal{L}_{rec}$ and $O\big(2sd|\mathcal{E}|\big)$ for $\mathcal{L}_{bpr}$.
(5) Lastly, \model~takes $O(snd|\mathcal{E}|)$ to estimate the gradients for the $d$-dimension hash codes.
Thus, thee total complexity in total is quadratic to the graph edge numbers, i.e., $|\mathcal{E}|$, which is common in GCN frameworks.
 % and actually acceptable for large bipartite graphs, which may dispel the concerns of the realistic training cost.


 \begin{table}[t]
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{0.2cm}
\centering
\notsotiny
\caption{Traing time complexity.}
\vspace{-0.05in}
\label{tab:train_time}
\setlength{\tabcolsep}{2mm}{
  \begin{tabular}{c | c | c | c | c }
\toprule
    {Graph Norm.}  & {Feat. Disp.}  & {Conv. \& Hash.}   & { Loss Comp.}  &{Grad. Est.} \\
\midrule[0.1pt]
    { $O(2|\mathcal{E}|)$} & {$O(\frac{2csK|\mathcal{E}|^2}{B})$} & {$O(\frac{2csL|\mathcal{E}|^2}{B})$} & { $O\big(2s(c$+$d)|\mathcal{E}|\big)$} & { $O(snd|\mathcal{E}|)$} \\
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[t]
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{0.2cm}
\centering
\footnotesize
\caption{Complexity of space and computation.}
\vspace{-0.05in}
\label{tab:prediction}
\setlength{\tabcolsep}{2.2mm}{
\begin{tabular}{c | c | c c}
\toprule
  ~          & {\footnotesize Space cost}   &  {\footnotesize \#FLOP} & {\footnotesize \#BOP}       \\
\midrule
\midrule
 {\scriptsize float32-based}      & {\scriptsize $32|\mathcal{V}_1 \cup \mathcal{V}_2|d$}       &   {\scriptsize $O\big(|\mathcal{V}_1| \cdot |\mathcal{V}_2| d\big)$}      &   {-}         \\
\midrule[0.1pt]
{\scriptsize \model}       & {\scriptsize $|\mathcal{V}_1 \cup \mathcal{V}_2| (d+32(L+1))$}    & {\scriptsize $O\big(4|\mathcal{V}_1| \cdot |\mathcal{V}_2| \big)$}            & {\scriptsize $O\big(|\mathcal{V}_1| \cdot |\mathcal{V}_2| d\big)$}    \\
\bottomrule
\end{tabular}}
\end{table}


% \vspace{0.05in}

% \subsubsection{\textbf{Hash Codes Space Cost.}}
\textbf{Hash codes space cost.}
As shown in Table~\ref{tab:prediction}, the total space cost of hash codes is {\small $O(|\mathcal{V}_1 \cup \mathcal{V}_2| (d+32(L+1)))$} bits, supposing that we use float32 for those rescaling factors in $L+1$ iterations.
Compared to the continuous embedding size, i.e., $32|\mathcal{V}_1 \cup \mathcal{V}_2|d$ bits, the theoretical size reduction ratio thus is:
\begin{equation}
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\label{eq:space}
ratio = \frac{32|\mathcal{V}_1 \cup \mathcal{V}_2|d}{|\mathcal{V}_1 \cup \mathcal{V}_2| (d+32(L+1))} = \frac{32d}{d+32(L+1)}.
\end{equation}
As we just explained, stacking too many iteration layers will incurring performance detriment~\cite{li2019deepgcns}. Hence, if $L\leq4$ and $d=1024$, \model~can achieve considerable size compression. 

\vspace{0.05in}

{\textbf{Online matching.}}
The original score formulation in Equation~(\ref{eq:inner_score}) contains $d$ floating-point operations (\#FLOPs).
As shown in Table~\ref{tab:prediction}, using Hamming distance matching can convert the most of floating-point arithmetics to binary operations (\#BOPs), with slightly more \#FLOPs for scalar computations, i.e., $4\ll d$.






==> app.tex <==
\appendix

\subsection{\textbf{Loss Landscape Visualization}}
\label{sec:visualization}
We simulate the optimization trajectories of learnable embeddings and visually compare the loss landscapes of non-hashing and hashing versions in Figure~\ref{fig:model}(a).
Specifically, we manually assign perturbations~\cite{nahshan2021loss, bai2020binarybert} to the embeddings on MovieLens dataset as: {\footnotesize$\emb{V}_x^{(l)} = \emb{V}_x^{(l)} \pm p \cdot$ $\overline{|{\emb{V}_x^{(l)}|}}$ $\cdot \emb{1}^{(l)}$}.
where {\footnotesize$\overline{|{\emb{V}_x^{(l)}|}}$} represents the absolute mean of entries in {\footnotesize$\emb{V}_x^{(l)}$} and perturbation magnitudes $p$ are from $\{0.01, \cdots, 0.50\}$. $\emb{1}$ is an all-one vector. 
For pairs of perturbed node embeddings, we plot their loss distribution accordingly.
As we can observe, the non-hashing version produces a flat loss surface, showing the local convexity.
On the contrary, the hashing counterpart has a bumping and complex loss landscape.




==> basic.tex <==
\section{Basic Implementation and Challenges}
\label{sec:baiscandchanlleges}
\subsection{Basic Implementation}
\label{sec:basic}
To differentiate from the conventional methodology~\cite{hashgnn,lsh,hashnet} and enable the \textit{topology-aware} hashing for the bipartite graphs, one straightforward implementation is to develop the embedding hashing for each \textit{iterative} graph convolution.
Specifically, let $\emb{V}^{(l)}$ $\in$ $\mathbb{R}^{(|\mathcal{V}_1| + |\mathcal{V}_2|) \times c}$ denote the \textit{continuous} embedding matrix computed in the $l$-th graph convolution iteration and it is initialized as $\emb{V}^{(0)}$.
$\emb{V}^{(l+1)}$ can be iteratively updated as follows:
\begin{equation}
\label{eq:conv}
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\emb{V}^{(l+1)} = (\emb{D}^{-\frac{1}{2}} \emb{A} \emb{D}^{-\frac{1}{2}} )\emb{V}^{(l)}, 
\end{equation}
where $\emb{D}$ is the (diagonal) degree matrix in which its diagonal entry denotes the node degree in $\emb{A}$. 
Then $\emb{Q}$ can be alternatively implemented as follow:
\begin{equation}
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{2pt}
\label{eq:basic}
\emb{Q}_{x}^{(l)} = \sign(\emb{V}_{x}^{(l)}), \text{ where } (\emb{Q}_{x}^{(l)})_i  = \left\{
\begin{aligned}
 &+ 1 &\text{  If } (\emb{V}_{x}^{(l)})_i \geq 0,\\
 & -1 &\text{  Otherwise.} 
\end{aligned}
\right.
\end{equation}
The outer subscript $i$ in $(\emb{V}_{x}^{(l)})_i$ denotes the $i$-th entry in embedding $\emb{V}_{x}$.
Equation~(\ref{eq:basic}) captures different depths of structural information with $l$ from 0 to the maximum depth $L$, and thus iteratively retains the latent node features related to each $\emb{V}^{(l)}$.
This \textit{topology-aware} implementation is different from the conventional methods~\cite{hashgnn,lsh,hashnet} that hash codes are computed \textit{only after} all the graph convolutions are processed, i.e., $\sign(\emb{V}_{x}^{(L)})$.
% Our experimental results {\cyk in~\cref{?}} demonstrate that this can already achieve effective performance improvement over the conventional couterparts.


\subsection{Challenges}
Despite the straightforwardness to capture the graph structural information for hashing, we argue that this trivial implementation contains several major inadequacies, which may lead to suboptimal performance.
Concretely, 
\begin{itemize}[leftmargin=*]

% \begin{figure}[tp]
% \begin{minipage}{0.5\textwidth}
% \includegraphics[width=3.5in]{figs/loss_curve.eps}
% \end{minipage} 
% \setlength{\abovecaptionskip}{0.2cm}
% \setlength{\belowcaptionskip}{0.2cm}
% \caption{Loss landscape visualization.}
% \label{fig:ste_loss}
% \end{figure}

\begin{figure*}[tp]
\hspace{-0.3cm}
\begin{minipage}{1\textwidth}
\includegraphics[width=7.1in]{figs/model_frame}
\end{minipage} 
\setlength{\abovecaptionskip}{0.2cm}
\setlength{\belowcaptionskip}{0.2cm}
\caption{Visualized loss landscape comparison and \model~model framework (best view in color).}
\label{fig:model}
\end{figure*}

\item \textbf{Feature erosion issue.}
Hashing via $\sign(\cdot)$ function will inevitably smooth the embedding feature informativeness, by converting each digit of continuous embeddings into the hamming space, i.e., \{-1,1\}$^d$, no matter what specific value it used to be.
Intuitively, if those \textit{informative} latent features are condensed and gathered in (relatively-small) sub-structures of embeddings, such simple hashing may thus more likely erode the most representative semantics in the original embeddings and generate undesired hash codes.
For example, compared to embeddings with condensed latent features, e.g., [0.97, 0.01, -0.01] and [0.81, 0.02, -0.01], embeddings such as [0.66, 0.43, -0.42] and [-0.45, -0.53, 0.22] tend to be more desirable and effective to indicate their feature uniqueness within all these three dimensions. 
However, current solutions lack certain mechanisms of explicitly avoiding information condensing to hedge the feature erosion in hashing.

\item \textbf{Coarse-grained matching score measurements.}
Because the hash codes are either -1 or 1, the matching scores (score formulation is introduced later in~\cref{sec:score_computation}) are thus coarse-grained, leading to the steep loss landscape for optimization.
We simulate the optimization trajectories of learnable embeddings and visually compare the loss landscapes of non-hashing and hashing versions in Figure~\ref{fig:model}(a).
Specifically, we manually assign perturbations~\cite{nahshan2021loss, bai2020binarybert} to the embeddings on MovieLens dataset (refer to~\cref{sec:exp_setup} for dataset details) as: {\footnotesize$\emb{V}_x^{(l)} = \emb{V}_x^{(l)} \pm p \cdot$ $\overline{|{\emb{V}_x^{(l)}|}}$ $\cdot \emb{1}^{(l)}$}.
where {\footnotesize$\overline{|{\emb{V}_x^{(l)}|}}$} represents the absolute mean of entries in {\footnotesize$\emb{V}_x^{(l)}$} and perturbation magnitudes $p$ are from $\{0.01, 0.02, \cdots, 0.50\}$. $\emb{1}$ is an all-one vector. 
For pairs of perturbed node embeddings, we plot their loss distribution accordingly.
As we can observe, the non-hashing version produces a flat loss surface, showing the local convexity.
On the contrary, the hashing counterpart has a bumping and complex loss landscape with coarse-grained score measurements.
% This is because both user and item embeddings are binarized into $\{0, 1\}^d$. Consequently, the computed loss is discretized, leading to the steep binarization loss curvature.

\item \textbf{Inaccurate gradient estimation.}
% As we have briefly introduced before, another non-negligible issue is the inaccurate gradient estimation.
As we have mentioned that $\sign(\cdot)$ is non-differentiable at 0 and produces the derivatives of 0 for anywhere else, which makes the \text{learning to hash} models hard to optimize.
Previous methods~\cite{bengio2013estimating,darabi2018bnn,sigmoid,RBCN} propose several approximation functions, e.g., $\tanh(\cdot)$, for $\sign(\cdot)$, and thus use their corresponding derivatives, e.g., $1$ $-$ $\tanh^2(\cdot)$, to estimate the gradients of $\sign(\cdot)$.
However, these approximation functions are usually \textit{visually similar} but not necessarily \textit{theoretically relevant}.
This may distract the main direction of the factual gradient for model optimization in forward and backward propagation, leading to performance degradation of bipartite matching.
\end{itemize}


% Hamming weight is the Hamming distance between this node to the origin.


==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/Yankai Chen.jpeg}}]{Yankai Chen} currently is a postdoctoral associate in Cornell University. 
He received his Ph.D. in The Chinese University of Hong Kong in 2023, M.S. degree from the University of Hong Kong in 2018, and B.S. degree from Nanjing University in 2016.
His research interests include artificial intelligence and machine learning for information retrieval, processing, and generation.
\end{IEEEbiography}

\vspace{-1cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/125_Yixiang_Fang.jpeg}}]{Yixiang Fang} is an associate professor at the School of Data Science in the Chinese University of Hong Kong, Shenzhen. He received the PhD degree from the University of Hong Kong in 2017 and worked as a postdoctoral researcher in the University of New South Wales from 2018 to 2020. His research interests mainly focus on the areas of graph data management, data mining, and graph learning. He serves as an editorial board member of Information Processing and Management.
\end{IEEEbiography}
\vspace{-1cm}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/yifei.jpeg}}]{Yifei Zhang} currently is the Ph.D. Student in Department of Computer Science and Engineering,The Chinese University of Hong Kong. He focuses on developing machine learning algorithms applied to graph-structured data. He work on generalized graph neural networks that are scalable to web-scale datasets, with applications in recommender systems, NLP, and IR systems.

\end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/125_Chenhao_Ma.jpeg}}]{Chenhao Ma}
is an assistant professor at the Chinese University of Hong Kong, Shenzhen. 
Prior to that, he was a postdoctoral fellow at the University of Hong Kong. 
He received his Ph.D. degree from Department of Computer Science in the University of Hong Kong in 2021.
His research interests mainly focus on large-scale data management and data mining, particularly graph data management with dense subgraph search, motif analysis, convex optimization and traffic data mining with trajectory outlier detection, traffic network weight completion.
\end{IEEEbiography}
\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/Yang_Hong.jpeg}}]{Yang Hong} currently is pursuing a Bachelor's degree at Ocean University of China. Her research interests are focused on data mining and machine learning, including areas such as graph neural networks, image segmentation, and related topics.
\end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/Irwin_King.jpeg}}]{Irwin King}
currently is the Chairman and a professor of Department of Computer Science and Engineering, and a former Associate Dean (Education), Faculty of Engineering at The Chinese University of Hong Kong.
He received the B.Sc. degree in engineering and applied science from the California Institute of Technology, Pasadena, CA, USA, and the M.Sc. and Ph.D. degrees in computer science from the University of Southern California, Los Angeles, CA. 
His broad range of research interests cover areas such as machine learning, social computing, AI, and data mining,
In these research areas, he has over 210 technical publications in journals and conferences. 
He is a Fellow of prestigious societies and associations, including the IEEE, INNS, AAIA, HKIE, and ACM Distinguished Member.
\end{IEEEbiography}

==> exp_hyper.tex <==
\subsection{\textbf{Study of Hyper-parameter Settings (RQ6)}}
\label{sec:hyper}

{\color{red} We put all settings in xxx? 1. lmbda and eposion!}





\subsubsection{\textbf{Impact of $\tau$.}}


\begin{table}[tbp]
\centering
\footnotesize
\caption{Recall@20 results (\%) \textit{w.r.t.} different $L$.}
\label{tab:layer}
\setlength{\tabcolsep}{1.3mm}{
\begin{tabular}{c | c | c | c | c | c | c }
\toprule
    $L$          & MovieLens & Gowalla & Pinterest & Yelp2018 & AMZ-Book & Dianping \\
\midrule[0.1pt]
  $L=1$          &{22.44}  &{16.21}  &{12.46}  &{5.25}  &{3.23}  &{9.57}  \\
  $L=2$          &{\textbf{22.86}}  &{16.73}  &{12.78}  &{5.51}  &{\textbf{3.48}}  &{10.66}  \\
  $L=3$          &{22.38}  &{\textbf{16.89}}  &{\textbf{13.12}}  &{\textbf{5.63}}  &{3.44}  &{10.72}  \\
  $L=4$          &{22.53}  &{16.38}  &{12.89}  &{5.53}  &{2.93}  &{\textbf{10.81}}  \\
\bottomrule
\end{tabular}
}
\end{table}

\subsubsection{Impact of \textbf{$\lambda_1$.}}
TBC





% \subsubsection{\textbf{Convolutional Hashing Depth $L$.}}
% We study how the convolutional hashing depth affects the performance by varying $L$ from 1 to 4.
% As shown in Table~\ref{tab:layer}, \model~achieves the best performance when $L$ is \{2, 3, 3, 3, 2, 4\} for all benchmarks.
% Generally, \model~model shares the common characteristics with the traditional graph-based models that usually set $L\leq4$~\cite{lightgcn,ngcf,kipf2016semi,graphsage}.
% This can effectively prevent the performance detriment caused by \textit{over-smoothing} problem~\cite{li2018deeper,li2019deepgcns}.
% Please notice that, in Table~\ref{tab:layer} we maximize the model performance by varying $L$. 
% Thus the results are different from Table~\ref{tab:full}, mainly because in Table~\ref{tab:full} we fix the $L$ and $d$ for a fair comparison.



% \begin{table}[tbp]
% % \setlength{\abovecaptionskip}{0cm}
% % \setlength{\belowcaptionskip}{0cm}
% \centering
% \footnotesize
% \caption{Recall@20 results (\%) \textit{w.r.t.} different $L$.}
% \label{tab:layer}
% \setlength{\tabcolsep}{1.3mm}{
% \begin{tabular}{c | c | c | c | c | c | c }
% \toprule
%     $L$          & Movie & Gowalla & Pinterest & Yelp2018 & AMZ-Book & Dianping \\
% \midrule[0.1pt]
%   $L=1$          &{22.44}  &{16.21}  &{12.46}  &{5.25}  &{3.23}  &{9.57}  \\
%   $L=2$          &{\textbf{22.86}}  &{16.73}  &{12.78}  &{5.51}  &{\textbf{3.48}}  &{10.66}  \\
%   $L=3$          &{22.38}  &{\textbf{16.89}}  &{\textbf{13.12}}  &{\textbf{5.63}}  &{3.44}  &{10.72}  \\
%   $L=4$          &{22.53}  &{16.38}  &{12.89}  &{5.53}  &{2.93}  &{\textbf{10.81}}  \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


% \subsubsection{\textbf{Cnvolution Dimension $c$.}}
% We verify the model performance with different convolution dimension $c$ in the range \{32, 64, 128, 256, 512\} and report the results in Table~\ref{tab:dimension}.
% As we can observe, increasing the dimension length is generally one way to improve the hash code informativeness.
% As for \model, the Top-N Hamming space retrieval quality is maximized when $c$ is \{512, 256, 512, 256, 256, 512\} for six graphs, respectively.
% Hence, it is flexible for the system users to select the dimension $c$ as the trade-off between the available resource consumption and target model performance.

% \begin{table}[h]
% \setlength{\abovecaptionskip}{0cm}
% \setlength{\belowcaptionskip}{0cm}
% \centering
% \footnotesize
% \caption{Recall@20 results (\%) \textit{w.r.t.} different $c$.}
% \label{tab:dimension}
% \setlength{\tabcolsep}{1.7mm}{
% \begin{tabular}{c | c | c | c | c | c | c}
% \toprule
%    c          & Movie & Gowalla & Pinterest & Yelp2018 & AMZ-Book & Dianping \\
% \midrule[0.1pt]
%   $c=32$           &{16.24}  &{11.98}  &{11.25}  &{4.57}  &{2.15}  &{7.58}  \\
%   $c=64$           &{18.84}  &{13.76}  &{12.08}  &{4.83}  &{2.39}  &{9.61}  \\
%   $c=128$          &{20.75}  &{14.65}  &{12.43}  &{5.22}  &{3.22}  &{10.12}  \\
%   $c=256$          &{22.86}  &\textbf{\textbf{16.73}}  &{12.78}  &\textbf{\textbf{5.51}}  &\textbf{\textbf{3.48}}  &{10.66}  \\
%   $c=512$          &\textbf{\textbf{22.82}}  &{16.02}  &\textbf{\textbf{12.80}}  &{5.46}  &{3.44}  &\textbf{\textbf{10.73}}  \\
% \bottomrule
% \end{tabular}}
% \end{table}



==> fd.tex <==
\subsection{Latent Feature Dispersion}


in other words, we seek to \textit{disperse the embedded features as one effective strategy to hedge the inevitable information loss caused by the numerical binarization and retain the feature uniqueness after binarization}. 

In singular value decomposition (SVD), singular values and corresponding singular vectors reconstruct the original matrix;
normally, large singular values can be interpreted to associate with major feature structures of the matrix~\cite{wei2018grassmann}. 
Hence, based on this observation, we can achieve feature dispersion via normalizing singular values for equalizing their respective contributions in constituting latent features.
To achieve this, Power Normalization~\cite{li2017second,koniusz2016higher,zhang2022spectral,quattoni2009recognizing} is one of the solutions that tackle related problems such as feature imbalance~\cite{koniusz2018deeper}.
Inspired by the recent approximation attempt~\cite{yu2020toward}, we introduce a light-weight feature dispersion techique in graph convolution as follows.
Concretely, let $\emb{I}$ denote the identity matrix, we start from generating a \textit{standard normal random vector} $\emb{p}^{(0)}$$\sim$$\mathcal{N}(\emb{0}, \emb{I})$ where $\emb{p}^{(0)}$ $\in$ $\mathbb{R}^{d}$.
Based on the embedding matrix to conduct feature dispersion, e.g., $\emb{E}$, we compute the desired \textbf{dispersing vector} $\emb{p}^{(h)}$ by iteratively performing $\emb{p}^{(h)} = \emb{E}^\mathsf{T}\emb{E}\emb{p}^{(h-1)}$.
Next we can obtain the projection matrix $\emb{P}$ of $\emb{p}$ via:
\begin{sequation}
\label{eq:projection}
\emb{P} = \frac{\emb{p}^{(h)}\emb{p}^{(h)^\mathsf{T}}}{||\emb{p}^{(h)}||_2^2}.
\end{sequation}%
Then we have the feature-dispersed representation matrix with the hyper-parameter $\epsilon$ $\in$ $(0,1)$ as follows:
\begin{sequation}
\widehat{\emb{E}} = \emb{E}(\emb{I} - \epsilon \emb{P}).
\end{sequation}%
Consequently, integrating the dispersed matrix $\widehat{\emb{E}}$, we propose the \textbf{feature-dispersed} graph convolution as follows:
\begin{sequation}
\label{eq:conv}
\widehat{\emb{E}}^{(l+1)} = (\emb{D}^{-\frac{1}{2}} \emb{A} \emb{D}^{-\frac{1}{2}} )\widehat{\emb{E}}^{(l)},  \text{ where } \widehat{\emb{E}}^{(0)} = \emb{E}^{(0)}(\emb{I} - \epsilon \emb{P}),
\end{sequation}%
where {\small $\emb{D}$} is the diagonal degree matrix of nodes in {\small $\emb{A}$}.
Equation~(\ref{eq:conv}) removes operations such as \textit{self-connection}, \textit{feature transformation}, and \textit{nonlinear activation} by following the observation in~\cite{lightgcn} mainly for architecture simplification. 
Note that we explicitly conduct this feature dispersion operation only at the initial step, i.e., {\small $\widehat{\emb{E}}^{(0)}$}, and, more importantly, such feature dispersion can be diffused via the multi-layers graph convolutions, i.e., from $l=0$ to $l=L$.
Thus, compare to the unprocessed embedding counterpart, e.g., {\small${\emb{E}}^{(l)}$}, embedding matrix {\small$\widehat{\emb{E}}^{(l)}$} at each layer presents a dispersed feature structure with a \textit{more balanced spectrum (distribution of singular values) in expectation}. 
We theoretically explain this by Theorem~\ref{tm:svd} in~\cref{sec:dispersion} and illustrate a visual comparison in Figure~\ref{fig:svd}.


% \begin{figure}[tp]
% \begin{minipage}{0.5\textwidth}
% % \hspace{-0.2in}
% \includegraphics[width=3.35in]{figs/svd}
% \end{minipage} 
% \setlength{\abovecaptionskip}{0.2cm}
% \setlength{\belowcaptionskip}{0.2cm}
% \vspace{-0.05in}
% \caption{Illustration of singular value distribution (sorted in descending order) on Dianping dataset: using feature dispersion technique can well balance the matrix spectrum.}
% \label{fig:svd}
% \end{figure} 


==> fd_analysis.tex <==
\begin{thm}[\textbf{Feature Dispersion}]
Let ${\emb{V}}^{(l)} = \emb{U}_1\emb{\Sigma}\emb{U}_2^\mathsf{T}$, where $\emb{U}_1$ and $\emb{U}_2$ are unitary matrices and descending singular value matrix $\emb{\Sigma} = \diag(\sigma_1, \sigma_2, \cdots, \sigma_c)$.  
Then $\mathbb{E}({\small\widetilde{\emb{V}}^{(l)}}) = \emb{U}_1\emb{\Sigma}\emb{\Sigma}_{\mu}\emb{U}_2^\mathsf{T}$ where $\emb{\Sigma}_{\mu} = \diag(\mu_1, \mu_2, \cdots, \mu_c)_{0<\mu_{1 \cdots c}<1}$ is in ascending order.
\end{thm}


\begin{proof}
We focus on comparing ({\small$\widetilde{\emb{V}}^{(0)}$, ${\emb{V}}^{(0)}$}), which can be easily popularized to any convolution layer, i.e., ({\small$\widetilde{\emb{V}}^{(l)}$, ${\emb{V}}^{(l)}$}). 
Conducting SVD decomposition on {\small${\emb{V}}^{(0)}$}, we have ${\emb{V}}^{(0)} = \emb{U}_1\emb{\Sigma}\emb{U}_2^\mathsf{T}$, where {\small$\emb{U}_1$} and {\small$\emb{U}_2$} are unitary matrices of singular vectors.
Then following {\small$\emb{p}^{(k)} = {\emb{V}^{(0)}}^\mathsf{T}\emb{V}^{(0)}\emb{p}^{(k-1)}$}, we shall have {\small $\emb{p}^{(k)} = ({\emb{V}^{(0)}}^\mathsf{T}\emb{V}^{(0)})^k\emb{p}^{(0)}$}.
Replacing {\small${\emb{V}}^{(0)}$} with its SVD decomposition, we get the following equation:
\begin{sequation}
\emb{p}^{(k)} = (\emb{U}_2\emb{\Sigma}^{2k}\emb{U}_2^\mathsf{T})\emb{p}^{(0)}.
\end{sequation}%
Then we transform the projection matrix in Equation~(\ref{eq:projection}) as follows:
\begin{sequation}
\begin{aligned}
\emb{P} = \frac{\emb{p}^{(k)} {\emb{p}^{(k)}}^\mathsf{T}}{{\emb{p}^{(k)}}^\mathsf{T} \emb{p}^{(k)}} & = \frac{(\emb{U}_2\emb{\Sigma}^{2k}\emb{U}_2^\mathsf{T})\emb{p}^{(0)} {\emb{p}^{(0)}}^\mathsf{T} (\emb{U}_2\emb{\Sigma}^{2k}\emb{U}_2^\mathsf{T})}
{{\emb{p}^{(0)}}^\mathsf{T} (\emb{U}_2\emb{\Sigma}^{2k}\emb{U}_2^\mathsf{T}) (\emb{U}_2\emb{\Sigma}^{2k}\emb{U}_2^\mathsf{T})\emb{p}^{(0)} } \\
 & = \emb{U}_2\emb{\Sigma}^{2k} \frac{\emb{U}_2^\mathsf{T}\emb{p}^{(0)} {\emb{p}^{(0)}}^\mathsf{T} \emb{U}_2} 
 {{\emb{p}^{(0)}}^\mathsf{T} \emb{U}_2\emb{\Sigma}^{4k}\emb{U}_2^\mathsf{T}\emb{p}^{(0)} }\emb{\Sigma}^{2k}\emb{U}_2^\mathsf{T}.
\end{aligned}
\end{sequation}%
Let $\emb{t} = \emb{U}_2^\mathsf{T}\emb{p}^{(0)}$, we can further simplify the above equation to:
\begin{sequation}
\emb{P} = \emb{U}_2 \emb{\Sigma}^{2k} \frac{ \emb{t} \emb{t}^\mathsf{T}}{\emb{t}^\mathsf{T}\emb{\Sigma}^{4k} \emb{t} }\emb{\Sigma}^{2k} \emb{U}_2^\mathsf{T}, 
 \text{ where scalar }  \emb{t}^\mathsf{T}\emb{\Sigma}^{4k} \emb{t} = \sum_{j=1}^c t_j^2 \sigma_j^{4k}.
\end{sequation}%
% Here {\small $\emb{t}^\mathsf{T}\emb{\Sigma}^{4k} \emb{t}$} is a scalar as:
% \begin{sequation}
% \emb{t}^\mathsf{T}\emb{\Sigma}^{4k} \emb{t} = \sum_{j=1}^c t_j^2 \sigma_j^{4k}.
% \end{sequation}%
Recalling that {\small $\widetilde{\emb{V}}^{(0)} = \emb{V}^{(0)}(\emb{I} - \epsilon \emb{P})$}, {\small $\mathbb{E}(\widetilde{\emb{V}}^{(0)}) = \emb{V}^{(0)} - \epsilon\cdot\mathbb{E}(\emb{V}^{(0)}\emb{P})$}.
Then we focus on the term {\small $\mathbb{E}(\emb{V}^{(0)}\emb{P})$} as follows:
\begin{sequation}
\mathbb{E}(\emb{V}^{(0)}\emb{P}) = \frac{1}{\emb{t}^\mathsf{T}\emb{\Sigma}^{4k} \emb{t}} \emb{U}_1 \emb{\Sigma}^{2k+1} \cdot \mathbb{E}(\emb{t} \emb{t}^\mathsf{T}) \cdot  \emb{\Sigma}^{2k} \emb{U}_2^\mathsf{T} 
\end{sequation}%
Since {\small$\emb{p}^{(0)}$$\sim$$\mathcal{N}(\emb{0}, \emb{I})$} and {\small $\emb{U}_2$} is a unitary matrix, thus {\small $\emb{t}$$\sim$$\mathcal{N}(\emb{0}, \emb{I})$}. 
This indices that each element of {\small $\emb{t}$}, e.g., {\small $t_j$ $\in$ $\emb{t}$}, is \textit{i.i.d.} random variable. Thus, {\small $\mathbb{E}({t}_j \cdot t_{k})=0$} for {\small$j\neq k$} and {\small $\mathbb{E}(\emb{t}\emb{t}^\mathsf{T})$} is a diagonal matrix, i.e., {\small $\mathbb{E}(\emb{t}\emb{t}^\mathsf{T})=\diag(t_1^2, t_2^2, \cdots, t_c^2)$}.
We then have:
\begin{sequation}
\mathbb{E}(\emb{V}^{(0)}\emb{P}) = \emb{U}_1 \cdot \diag \big(\frac{\sigma_1 t_1^2 \sigma_1^{4k}}{\sum_{j=1}^c t_j^2 \sigma_j^{4k}},  \cdots,  \frac{\sigma_c  t_c^2\sigma_c^{4k}}{\sum_{j=1}^c t_j^2 \sigma_j^{4k}}\big) \cdot \emb{U}_2^\mathsf{T}.
\end{sequation}%
Therefore, 
\begin{sequation}
\mathbb{E}(\widetilde{\emb{V}}^{(0)}) = \emb{U}_1 \cdot \diag \big( \sigma_1 - \epsilon \frac{\sigma_1 t_1^2 \sigma_1^{4k}}{\sum_{j=1}^c t_j^2 \sigma_j^{4k}},  \cdots,  \sigma_c - \epsilon \frac{\sigma_c  t_c^2\sigma_c^{4k}}{\sum_{j=1}^c t_j^2 \sigma_j^{4k}} \big)  \cdot \emb{U}_2^\mathsf{T}.
\end{sequation}%
Let {\small $\mu_k = 1 - \epsilon \frac{t_k^2\sigma_k^{4k}}{\sum_{j=1}^c t_j^2 \sigma_j^{4k}}$}, with {\small $\epsilon$ $\in$ $(0,1)$}, obviously, {\small $0<\mu_k<1$}. 
Furthermore, {\small $\forall k_1$ $\geq$ $k_2$}, we have:
\begin{sequation}
\label{eq:increase}
\resizebox{1\linewidth}{!}{$
\displaystyle
\mu_{k_1} - \mu_{k_2} = \epsilon \mathbb{E}(\frac{t_{k_1}^2\sigma_{k_1}^{4k}}{\sum_{j=1}^c t_j^2 \sigma_j^{4k}} - \frac{t_{k_2}^2\sigma_{k_2}^{4k}}{\sum_{j=1}^c t_j^2 \sigma_j^{4k}}) \geq \epsilon\sigma_{k_1}^{4k} \cdot \mathbb{E} (\frac{t_{k_1}^2 - t_{k_2}^2}{\sum_{j=1}^c t_j^2 \sigma_j^{4k}}) =0,
$}
\end{sequation}%
as {\small $\sigma_{k_2}^{4k} \geq \sigma_{k_1}^{4k}$}, and $t_{k_1}$ and $t_{k_2}$ are \textit{i.i.d.} random variables with same normal distribution.
Equation~(\ref{eq:increase}) proves that {\small $\mu_k$} is \textit{monotone non-decreasing} in expectation, which completes the proof.
\end{proof}



==> method_fd.tex <==
\subsection{Latent Feature Dispersion}
\label{sec:fd}

To tackle the feature erosion issue, we seek to disperse the embedded features as one effective strategy to hedge the inevitable information loss caused by numerical binarization.
From the perspective of singular value decomposition (SVD), singular values and corresponding singular vectors reconstruct the original matrix;
normally, large singular values can be interpreted to associate with \textit{major feature structures} of the matrix~\cite{wei2018grassmann}. 
Since we want to avoid condensing and gathering informative features in (relatively small) embedding sub-structures, it is natural to bridge the target by working on these singular values.
Hence, based on this intuition, we aim to \textit{normalize singular values for equalizing their respective contributions in constituting latent features}.
To achieve this, Power Normalization~\cite{koniusz2016higher,zhang2022spectral} is one of the solutions that tackle related problems such as feature imbalance~\cite{koniusz2018deeper}.
Inspired by the recent approximation attempt~\cite{yu2020toward}, we now introduce a lightweight feature dispersion technique in graph convolution as follows.


Concretely, let $\emb{I}$ denote the identity matrix, we start from generating a \textit{standard normal random vector} $\emb{p}^{(0)}$$\sim$$\mathcal{N}(\emb{0}, \emb{I})$ where $\emb{p}^{(0)}$ $\in$ $\mathbb{R}^{c}$.
Based on the embedding matrix to conduct feature dispersion, e.g., let $\emb{V}= \emb{V}^{(0)}$, we compute the desired \textbf{dispersing vector} $\emb{p}^{(k)}$ by iteratively performing $\emb{p}^{(k)} = \emb{V}^\mathsf{T}\emb{V}\emb{p}^{(k-1)}$.
The iteration for generating dispersing vectors is independent of the graph convolution iterations\footnote{\scriptsize In our work, we set $K \leq L$ mainly to enable the associated complexity of dispersing vector generation is upper bounded by the graph convolution complexity.}.
We have the projection matrix $\emb{P}$ of $\emb{p}^{(K)}$ via:
\begin{sequation}
\label{eq:projection}
\emb{P} = \frac{\emb{p}^{(K)}\emb{p}^{(K)^\mathsf{T}}}{||\emb{p}^{(K)}||_2^2}.
\end{sequation}%
Then we have the feature-dispersed representation matrix with the hyper-parameter $\epsilon$ $\in$ $(0,1)$ as follows:
\begin{sequation}
\label{eq:disperse}
\widetilde{\emb{V}} = \emb{V}(\emb{I} - \epsilon \emb{P}).
\end{sequation}%
Consequently, integrating the dispersed matrix $\widetilde{\emb{V}}$, we have the \textbf{feature-dispersed} graph convolution as:
\begin{sequation}
\label{eq:fdconv}
\widetilde{\emb{V}}^{(l+1)} = (\emb{D}^{-\frac{1}{2}} \emb{A} \emb{D}^{-\frac{1}{2}} )\widetilde{\emb{V}}^{(l)},  \text{ where } \widetilde{\emb{V}}^{(0)} = \emb{V}^{(0)}(\emb{I} - \epsilon \emb{P}).
\end{sequation}%
Note that we explicitly conduct this feature dispersion operation one time only at the initial step, i.e., {\small $\widetilde{\emb{V}}^{(0)}$}, and, more importantly, such feature dispersion can be diffused via the multi-layer graph convolutions from $0$ to $L$.
Compare to the unprocessed embedding counterpart, e.g., {\small${\emb{V}}^{(l)}$}, embedding matrix {\small$\widetilde{\emb{V}}^{(l)}$} at each layer presents a dispersed feature structure with a \textit{more balanced distribution of singular values in expection}. 
We formally explain this as follows: 
\vspace{-0.05in}
\begin{thm}[\textbf{Feature Dispersion}]
\label{tm:svd}
Let ${\emb{V}}^{(l)} = \emb{U}_1\emb{\Sigma}\emb{U}_2^\mathsf{T}$, where $\emb{U}_1$ and $\emb{U}_2$ are unitary matrices and descending singular value matrix $\emb{\Sigma} = \diag(\sigma_1, \sigma_2, \cdots, \sigma_c)$.  
Then $\mathbb{E}({\small\widetilde{\emb{V}}^{(l)}}) = \emb{U}_1\emb{\Sigma}\emb{\Sigma}_{\mu}\emb{U}_2^\mathsf{T}$ where $\emb{\Sigma}_{\mu} = \diag(\mu_1, \mu_2, \cdots, \mu_c)_{0<\mu_{1 \cdots c}<1}$ is in ascending order.
\end{thm}

% \begin{figure}[tp]
% \hspace{-0.5cm}
% \begin{minipage}{0.5\textwidth}
% \includegraphics[width=3.5in]{figs/fd}
% \end{minipage} 
% \setlength{\abovecaptionskip}{0.2cm}
% \setlength{\belowcaptionskip}{0.2cm}
% \caption{An example matrix spectrum on Dianping dataset (singular values are in the descending order).}
% \label{fig:svd}
% \end{figure}
\vspace{-0.05in}
Intuitively, given the same orthonormal bases, compared to {\footnotesize$\emb{V}^{(l)}$}, it is harder in expectation to reconstruct {\footnotesize$\widetilde{\emb{V}}^{(l)}$} with informative features being dispersed out in larger matrix sub-structures.
This eventually provides the functionality to hedge the information loss in numerical binarization. 
% We attach the theorem proof in~\cref{sec:discuss} and evaluate the module effectiveness later in~\cref{sec:ablation}.
We attach the theorem proof in Appendix C and evaluate the module effectiveness later in~\cref{sec:ablation}.


